A Max-Min Entropy Framework for Reinforcement Learning

In this paper, we propose a max-min entropy framework for reinforcement learning (RL) to overcome the limitation of the soft actor-critic (SAC) algorithm implementing the maximum entropy RL in model-free sample-based learning. Whereas the maximum entropy RL guides learning for policies to reach states with high entropy in the future, the proposed max-min entropy framework aims to learn to visit states with low entropy and maximize the entropy of these low-entropy states to promote better exploration. For general Markov decision processes (MDPs), an efficient algorithm is constructed under the proposed max-min entropy framework based on disentanglement of exploration and exploitation. Numerical results show that the proposed algorithm yields drastic performance improvement over the current state-of-the-art RL algorithms.

==> setup.tex <==
\pagestyle{myheadings}

\renewcommand{\thefootnote}{\fnsymbol{footnote}}
\setcounter{footnote}{1}
%\input /user/ltong/tex/macros/macros.tex
\makeatletter
\newdimen{\captionwidth}
\long\def\@makecaption#1#2{%
\captionwidth 1.0\hsize% use current value of \hsize
\vskip 10pt%
\setbox\@tempboxa\hbox{#1: #2}%
  \ifdim \wd\@tempboxa >\captionwidth%
    \setbox\@tempboxa\hbox{#1:\hspace*{.5em}}%
    \hfil\parbox{\captionwidth}{\raggedright\hangindent \wd\@tempboxa%
    \hangafter=1\unhbox\@tempboxa#2}\hfill%
%  \else \hbox to\captionwidth{\hfil\box\@tempboxa\hfil}%
  \else\centerline{\box\@tempboxa}%
  \fi
}
\makeatother
%\input epsf
\def\scalefig#1{\epsfxsize #1\textwidth}
\makeatletter
\font\hmed=cmr10 at 10pt
\def\ps@plain{\let\@mkboth\@gobbletwo
     \def\@oddhead{}\def\@oddfoot{\hmed\hfil
 / \footernote\ / \qquad \thepage}
\def\@evenhead{}\def\@evenfoot{\hmed
\thepage\qquad /  / \footernote\ \hfil }
}
\def\footernote{{\it \small }} 

\makeatother

\makeatletter
\newtheorem{theorem}{Theorem}
\newtheorem{corollary}{Corollary}
\newtheorem{lemma}{Lemma}
\newtheorem{definition}{Definition}
\newtheorem{problem}{Problem}
\newtheorem{assumption}{A}
\newtheorem{properties}{Properties}
\newtheorem{conjecture}{Conjecture}
\newtheorem{criterion}{Criterion}
\newtheorem{proposition}{Proposition}
\newtheorem{remark}{Remark}
\newtheorem{notation}{Notation}
\newtheorem{derivation}{Derivation}
%\bibliographystyle{ieee}

\renewcommand\baselinestretch{1.0}

%\footernote{\protect\tiny Submitted to IEEE Transactions On Signal Processing}












==> viewgr.tex <==
%
%  vgmac.tex -- viewgraph macros for tex
%
%               vgmac is intended for use with the 12pt article style.
%               The commands currently suported are:
%
%               Format commands:
%                  \horizfmt - horizontally formatted vg's
%                  \vertfmt  - vertically     "       "     (default)
%
%               Fonts:
%                  \bodyfont - std. font for body of vg     (default)
%                  \bodysmall - small font for body of vg
%                  \bodybold -  bold   "    "   "   "   "
%                  \bodyital - italic  "    "   "   "   "
%                  \titlefont - large font used for vg titles
%
%               Pagestyles:
%                  vgdatelabel - footer with left-justified filename
%                                and runtime, right-justified
%                                pagenumber                 (default)
%                  vgemptydatelabel - footer with left-justified runtime
%                                     and right-justified file name
%
%                 *N.B. if the filenames are relative to the current
%                       directory, the true path will appear in the footer
%                       only if the user has the following alias for latex:
%
%                       alias latex 'latex \\def\\dirname\{`pwd`\}\\input '
%
%               Page Initialization:
%                  \invg#1 - command to input a new viewgraph file.
%                            vg files are each assumed to contain a
%                            single vg.  #1 is as for the \input command.
%                  \newvgtitle#1 - command to initialize a vg with
%                                  title #1
%                  \newvgempty   - command to initialize a vg with no title
%
%                 *N.B. The first command in each vg file must be
%                       either \newvgtitle or \newvgempty
%
%               Text Layout:
%                  \leftitem#1 -      a bulleted, hanging indentation,
%                                     raggedright paragraph with contents #1
%                  \indentedpar#1#2 - a centered narrow paragraph #2
%                                     with bold label #1
%                  \bigskip -         has been redefined with infinite stretch
%
%                 *N.B. It is recommended that items in the viewgraph
%                       be seperated with \bigskip's
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
%  $Header: /user2/marcg/tex/macros/RCS/vgmac.tex,v 1.3 1992/02/11 01:20:42 marcg Exp marcg $
%
%  $Log: vgmac.tex,v $
%  Revision 1.3  1992/02/11  01:20:42  marcg
%  added \bodytiny and \bodytinyital
%
%  Revision 1.2  1991/03/19  01:10:40  marcg
%  added \par to \indentedpar
%
%  Revision 1.1  91/02/22  10:10:13  marcg
%  Initial revision
%
%
%  marcg, 1/22/91, Initial commented version
%  marcg, 1/29/91, Improved footer filename handling
%  marcg, 2/11/91, local definition of \xxvpt
%  marcg, 2/20/91, changed def of indentedpar to use current value of
%                  \textwidth
%  marcg, 2/21/91, replaced definition of \xxvpt with initialization
%                  of \@xxvpt for relative independence from
%                  lfonts.tex.  Dick mentioned that the rascals
%                  version of lfonts uses 25pt fonts in \xxvpt, while
%                  many other systems use 20pt fonts there.
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\typeout{vgmac package, $Revision: 1.3 $, $Date: 1992/02/11 01:20:42 $}
%
% page layout and fonts
%
\oddsidemargin 0truein \topmargin -.25truein \headheight 0pt
\headsep 0pt \topskip 0pt
\renewcommand\baselinestretch{1.1}
\def\magstepsix{2985}
\def\magstepseven{3583}
\font\titlefont = cmssbx10 scaled\magstep5
\font\bodyfont = cmss10 scaled\magstep4
\font\bodysmall = cmss10 scaled\magstep3
\font\bodytiny = cmss10 scaled\magstep2
\font\bodytinyital = cmssi10 scaled\magstep2
\font\bodybold = cmssbx10 scaled\magstep4
\font\bodyital = cmssi10 scaled\magstep4
\leftmargini .75 truein \rightmargin .5 truein
\leftmarginii .75 truein
\leftmarginiii .75 truein
\leftmarginiv .75 truein
\itemsep 15pt plus 20pt minus 5pt
\def\bigskip{\vskip .9em plus 1fil minus .15em}
%
%  format comands
%
\def\horizfmt{\textwidth 9.50truein \textheight 7.0truein
\special{landscape}}
%\special{header=/user/young/tex/macros/YMCAlandscapevglogo.ps}
\def\vertfmt{\textwidth 6.5truein \textheight 9.50truein}
%\special{header=/user/young/tex/macros/YMCAvglogo.ps}
%
%  \newvgtitle starts a new titled viewgraph
%  \newvgempty starts a new untitled viewgraph
%
\def\newvgtitle#1{\begin{center} \Huge\titlefont #1 \\[-.2em]
\rule{\textwidth}{2pt}
\end{center}
\LARGE\bodyfont
\raggedright
\parindent 0pt
}
\def\newvgempty{\LARGE\bodyfont\raggedright\parindent 0pt}
%
%  \invg inputs a viewgraph file and sets up footer filename as
%  follows:
%     filename starting with '/' --> footer contains filename
%     otherwise --> footer contains filename prepended with \dirname
%                   if it exists.
%
\def\invg#1{\clearpage\def\vgfilename{#1}
  \getinit{#1}
  \gdef\vglabelname{%
    \if\initchar/\else%
      \expandafter\ifx\csname dirname\endcsname\relax%
      \else\expandafter\badBgone\dirname\relax/\fi\fi%
        \expandafter\badBgone\vgfilename\relax.tex}%
\input #1}
%
%  \getinit sets the global variable \initchar to the first token of
%  its argument.
%
\newif\ifreadone  % used by \firstchar
\def\getinit#1{\firstchar#1\relax}
\def\firstchar#1{%
  \ifreadone\relax\else \gdef\initchar{#1}\readonetrue\fi%
  \if #1\relax\readonefalse\let\next=\relax%
  \else\let\next=\firstchar\fi%
  \next%
}
%
%  \leftitem yields a left justified paragraph with a bullet
%
\def\leftitem#1{\medskip
\setbox1\hbox{$\bullet$\hskip 1em}
\leavevmode\hangindent\wd1\hangafter1{\box1 #1\par}}
%
%  \indentedpar yields an narrow centered paragraph, #2, with label #1
%  The idea is to make the lines of the parbox maximally long with
%  no hyphenation and a raggedright.  The argument of the parbox used
%  to be '\raggedright #2'
%
\newdimen\indparind\indparind 3em
\newdimen\indparwd
\long\def\indentedpar#1#2{\indparwd\textwidth\advance\indparwd by -2\indparind
  {\bodybold #1:}\hfil\break
  \null\hskip\indparind\parbox[t]{\indparwd}{%
\linepenalty 10000\hyphenpenalty 10000\rightskip 0pt plus3em{#2}}\par}
%
%  makeatletter required for badBgone, ps@vgdatelabel,
%  ps@vgemptydatelabel, xxvpt
%
\makeatletter
\def\badBgone#1{\toks0={#1}\expandafter\if\the\toks0\relax%
    \let\next=\relax\else%
    \expandafter\if\the\toks0_\_%
    \else\expandafter\if\the\toks0&\&%
    \else\expandafter\if\the\toks0$\$%
    \else\expandafter\if\the\toks0^\^{ }%
    \else\expandafter\if\the\toks0<$\m@th <$%
    \else\expandafter\if\the\toks0>$\m@th >$%
    \else\expandafter\if\the\toks0##{$\m@th\sharp$}%
    \else\expandafter\if\the\toks0\noexpand{{$\m@th\{$}%
    \else\expandafter\if\the\toks0\noexpand}{$\m@th\}$}%
    \else\expandafter\if\the\toks0\noexpand%\%%
    \else\the\toks0\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi%
    \let\next=\badBgone\fi%
    \next}%
%
%
\def\ps@vgdatelabel{\let\@mkboth\@gobbletwo
     \def\@oddhead{}
     \newdimen\mydimen \mydimen=\textwidth
     \divide\mydimen by 2
     \newcount\hours \hours=\time \divide\hours by 60
     \newcount\minutes \minutes=\hours \multiply\minutes by
                           -60 \advance\minutes by\time
     \def\@oddfoot{\hbox to\textwidth{\footnotesize\sl\today, \the\hours:%
         \ifnum\minutes<10 0\fi\the\minutes\ --- %
         \vglabelname\hfill\rm\thepage}}
     \def\@evenhead{}\let\@evenfoot\@oddfoot%
     }
%
%
\def\ps@vgemptydatelabel{\let\@mkboth\@gobbletwo
     \def\@oddhead{}
     \newdimen\mydimen \mydimen=\textwidth
     \divide\mydimen by 2
     \newcount\hours \hours=\time \divide\hours by 60
     \newcount\minutes \minutes=\hours \multiply\minutes by
                           -60 \advance\minutes by\time
     \def\@oddfoot{\hbox to\mydimen{\footnotesize\sl\today, \the\hours:%
         \ifnum\minutes<10 0\fi\the\minutes\hfill}\hss%
         \hbox to\mydimen{\quad\footnotesize\sl\hfill%
         \vglabelname\hss}}
     \def\@evenhead{}\let\@evenfoot\@oddfoot%
     }
%
%  xxvpt is called by \Huge at 12pt in article style, so we initialize
%  @xxvpt to load in sanserif fonts.  This allows us to override the
%  definition in xxvpt independent of the machine type.  This whole
%  exercise is to fix some of my math macros that use \sf
%
%\@getfont\psf\sffam\@xxvpt{\@mss\@magscale5}\normalsize
\makeatother
%
%  default is vertical format and vgdatelabel pagestyle
%
\vertfmt
\pagestyle{vgdatelabel}

